Physics-Informed Graph Neural Network Surrogates for Turbulent Nanoparticle Dispersion in Dental Clinical Environments

Dental aerosol procedures produce sub-50 micrometre nuclei that can remain airborne for long periods in enclosed clinics, creating pathways for airborne pathogen transmission. Reynolds-Averaged Navier-Stokes (RANS) simulations with Euler-Lagrange particle tracking capture this transport accurately but require very long run times per scenario, which precludes real-time clinical decision support in 3D. We present the Eulerian-Lagrangian Graph Interaction Network (ELGIN), a physics-informed graph surrogate that jointly predicts carrier-flow dynamics on the OpenFOAM polyhedral mesh and the per-parcel motion of the polydisperse spray cloud. ELGIN couples a multi-head Graph Transformer with Jacobi-preconditioned learnable pressure projection and a turbulence-closure head to a sigmoid-gated Lagrangian Interaction Network through differentiable inverse-distance mesh-parcel coupling, and advances parcels with a symplectic Stormer-Verlet integrator. A four-stage physics-informed curriculum stabilises 260-step autoregressive rollouts without gradient explosion. A parameter sweep with foam-extend 4.1 OpenFOAM reactingParcelFoam across clinically relevant ventilation rates and handpiece spray speeds provides CFD ground truth. This article reports a single-case demonstration in which both ELGIN and a Lagrangian-only baseline (M0) are trained and evaluated on Sweep_Case_03 of a twenty-case sweep; full 16/2/2 retraining is in progress and will replace all reported metrics. On this case, ELGIN tracks the foam-extend particle cloud much more closely than M0: mean parcel displacement error falls from 19.56% to 16.20% of room width and cloud radius-of-gyration error from 9.85% to 6.58%. A 26-second rollout completes in ~64 s on a 4 GB GPU, approximately 37x faster than the foam-extend reference pipeline, toward per-appointment infection-risk screening once the multi-case checkpoint is in place.

==> latexmkrc <==
# ---------------------------------------------------------------------------
# Overleaf + bibunits notes
# ---------------------------------------------------------------------------
# Supporting Information (xr): if a separate main uses \usepackage{xr} and
# \externaldocument{paper}, keep paper.aux beside paper.tex when building
# that project variant. If ?? remain, use paper_si_xref_stubs.tex fallback.
#
# With \usepackage{bibunits} and \begin{bibunit}...\putbib...\end{bibunit},
# BibTeX must run on bu1, bu2, ... (not only on the main job name). Overleaf's
# latexmk usually does this automatically after a *clean, successful* PDF build.
#
# If you never see bu1.bbl / bu2.bbl:
#   • Menu → Compiler: pdfLaTeX (not LuaLaTeX/XeLaTeX unless you intend it).
#   • Do NOT use biblatex/biber with bibunits.
#   • Fix all LaTeX errors first; otherwise bu*.aux may not be written.
#   • Menu → Recompile from scratch, then open:
#     Menu → Logs and output files → look for bu1.bbl, bu2.bbl (download).
#
# Local fallback (Windows): run .\compile-bibunits.ps1 in this folder
# (requires full TeX + all figures so pdflatex completes pass 1).
#
# Optional manual sequence (two-document workflow): Main = paper.tex, compile
# x2, then main = supporting_information.tex, compile x2.
# ---------------------------------------------------------------------------

# Encourage latexmk to keep trying BibTeX when .aux files change (harmless).
$bibtex_use = 2;

